Gallium Anomaly: Critical View from the Global Picture of $\nu_{e}$ and $\bar\nu_{e}$ Disappearance

The significance of the Gallium Anomaly, from the BEST, GALLEX, and SAGE radioactive source experiments, is quantified using different theoretical calculations of the neutrino detection cross section, and its explanation due to neutrino oscillations is compared with the bounds from the analyses of reactor rate and spectral ratio data, $\beta$-decay data, and solar neutrino data. In the 3+1 active-sterile neutrino mixing scheme, the Gallium Anomaly is in strong tension with the individual and combined bounds of these data sets. In the combined scenario with all available data, the parameter goodness of fit is below 0.042%, corresponding to a severe tension of 4-5$\sigma$, or stronger. Therefore, we conclude that one should pursue other possible solutions beyond short-baseline oscillations for the Gallium Anomaly. We also present a new global fit of $\nu_e$ and $\bar\nu_e$ disappearance data, showing that there is a 2.6-3.3$\sigma$ preference in favor of short-baseline oscillations, which is driven by an updated analysis of reactor spectral ratio data.

==> tables/rat-gal-pgf-chi.tex <==
\begin{tabular}{c|c|c|c|c}
&
HM
&
HKSS
&
EF
&
KI
\\
\hline
Ground State
&
$7.2$
&
$5.4$
&
$9.1$
&
$11.9$
\\
\hline
Bahcall
&
$10.9$
&
$8.9$
&
$12.9$
&
$16.3$
\\
\hline
Kostensalo
&
$9.6$
&
$7.5$
&
$11.5$
&
$15.3$
\\
\hline
Semenov
&
$15.1$
&
$12.6$
&
$17.0$
&
$22.5$
\\
\hline
\end{tabular}


==> tables/rat-gal-pgf-gof.tex <==
\begin{tabular}{c|c|c|c|c}
&
HM
&
HKSS
&
EF
&
KI
\\
\hline
Ground State
&
$2.8\%$
&
$6.8\%$
&
$1.1\%$
&
$0.26\%$
\\
\hline
Bahcall
&
$0.42\%$
&
$1.2\%$
&
$0.16\%$
&
$0.029\%$
\\
\hline
Kostensalo
&
$0.83\%$
&
$2.4\%$
&
$0.31\%$
&
$0.049\%$
\\
\hline
Semenov
&
$0.052\%$
&
$0.18\%$
&
$0.02\%$
&
$0.0013\%$
\\
\hline
\end{tabular}

